Closed-loop Position Control of a Pediatric Soft Robotic Wearable Device for Upper Extremity Assistance

This work focuses on closed-loop control based on proprioceptive feedback for a pneumatically-actuated soft wearable device aimed at future support of infant reaching tasks. The device comprises two soft pneumatic actuators (one textile-based and one silicone-casted) actively controlling two degrees-of-freedom per arm (shoulder adduction/abduction and elbow flexion/extension, respectively). Inertial measurement units (IMUs) attached to the wearable device provide real-time joint angle feedback. Device kinematics analysis is informed by anthropometric data from infants (arm lengths) reported in the literature. Range of motion and muscle co-activation patterns in infant reaching are considered to derive desired trajectories for the device's end-effector. Then, a proportional-derivative controller is developed to regulate the pressure inside the actuators and in turn move the arm along desired setpoints within the reachable workspace. Experimental results on tracking desired arm trajectories using an engineered mannequin are presented, demonstrating that the proposed controller can help guide the mannequin's wrist to the desired setpoints.

==> state_machine_2.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3.cm,
                    semithick]
  \tikzstyle{every state}=[rectangle, fill=white,draw=none,text=black,minimum size=17pt]
% \tikzstyle{vertex}=[rectangle,fill=black!25,minimum size=17pt,inner sep=0pt]

  \node[state] (A) [rectangle,draw]              {Regrasp CW};
  \node[state, accepting]         (B) [rectangle,draw] [right of=A] {Tip};
  \node[state]         (C) [rectangle,draw] [below right of=B] {Regrasp CCW};
  \node[initial,state]         (E) [rectangle,draw] [below right of=A] {Touchdown};
  \path (A) edge              	node [black, pos=0.5] {$\overline{\mathbb{A}_0}$} (B)
        (B) edge   [bend left]            	node [black, pos=0.5, right] {$\overline{\mathbb{B}_0}$} (C)
                (C) edge   [bend left]            	node [black, pos=0.5, right] {$\overline{\mathbb{C}_0}$} (B)
%         (B) edge             	node [black, pos=0.5, left] {$\overline{\mathbb{B}_1}$} (E)
        (E) edge           	node  [black, pos=0.5, right] {$\overline{\mathbb{D}_0}$}  (A);
%         (E) edge   [bend left]          	node  [black, pos=0.5, left] {$\overline{\mathbb{A}_1}$}  (A);
\end{tikzpicture}

==> state_machine_tkz.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=4.cm,
                    semithick]
  \tikzstyle{every state}=[rectangle, fill=white,draw=none,text=black,minimum size=15pt]
% \tikzstyle{vertex}=[rectangle,fill=black!25,minimum size=17pt,inner sep=0pt]

  \node[initial,state] (A) [rectangle,draw]              {Tilt CCW $\theta_{0_{MAX}}$};
  \node[state]         (B) [rectangle,draw] [right of=A] {Dynamic Grasp: Lift};
  \node[state,accepting]         (E) [rectangle,draw] [below right of=A] {Dynamic Grasp: Slowdown};
  \path (A) edge  [bend left]            	node [black, pos=0.5 ] {$\mathbb{A}_0$} (B)

        (B) edge      [bend left]       	node [black, pos=0.5, left] {$\mathbb{B}_1$} (E)
   %     (E) edge   [bend right]          	node  [black, pos=0.5, left] {$\mathbb{D}_0$}  (A)
        (A) edge   [bend right]          	node  [black, pos=0.5, left] {$\mathbb{A}_1$}  (E);
\end{tikzpicture}
